Improved Parallel Cache-Oblivious Algorithms for Dynamic Programming and Linear Algebra

Emerging non-volatile main memory (NVRAM) technologies provide byte-addressability, low idle power, and improved memory-density, and are likely to be a key component in the future memory hierarchy. However, a critical challenge in achieving high performance is in accounting for the asymmetry that NVRAM writes can be significantly more expensive than NVRAM reads. In this paper, we consider a large class of cache-oblivious algorithms for dynamic programming (DP) and linear algebra, and try to reduce the writes in the asymmetric setting while maintaining high parallelism. To achieve that, our key approach is to show the correspondence between these problems and an abstraction for their computation, which is referred to as the $k$-d grids. Then by showing lower bound and new algorithms for computing $k$-d grids, we show a list of improved cache-oblivious algorithms of many DP recurrences and in linear algebra in the asymmetric setting, both sequentially and in parallel. Surprisingly, even without considering the read-write asymmetry (i.e., setting the write cost to be the same as the read cost in the algorithms), the new algorithms improve the existing cache complexity of many problems. We believe the reason is that the extra level of abstraction of $k$-d grids helps us to better understand the complexity and difficulties of these problems. We believe that the novelty of our framework is of interests and leads to many new questions for future work.

==> app-dp.tex <==
\section{Parenthesis Recurrence}\label{sec:parenthesis}

The Parenthesis recurrence solves the following problem: given a linear sequence of objects, an associative binary operation on those objects, and the cost of performing that operation on any two given (consecutive) objects (as well as all partial results), the goal is to compute the min-cost way to group the objects by applying the operations over the sequence.
Let $D_{i,j}$ be the minimum cost to merge the objects indexed from $i+1$ to $j$ (1-based), the recurrence for $0\le i<j\le n$ is:
\[D_{i,j}=\min_{i<k<j}\{D_{i,k}+D_{k,j}+w(i,k,j)\}\]
where $w(i,k,j)$ is the cost to merge the two partial results of objects indexed from $i+1$ to $k$ and those from $k+1$ to $j$.
Here the cost function is only decided by a constant-size input associated to indices $i$, $j$ and $k$.
$D_{i,i+1}$ is initialized, usually as 0.
The applications of this recurrence include the matrix chain product, construction of optimal binary search trees, triangulation of polygons, and many others shown in~\cite{CLRS,galil1992dynamic,galil1994parallel,yao1980efficient}.

The computation of this recurrence (without considering dependencies) is a (1/3)-full \kdcomp{3}, which has the same lower bound shown in Corollary~\ref{thm:mm}.

The divide-and-conquer algorithm that computes this recurrence is usually hard to describe (e.g., it takes several pages in~\cite{chowdhury2016autogen,itzhaky2016deriving} although they also describe their systems simultaneously).
We claim that under the view of our \ourcomp{s}, this algorithm is conceptually as simple as the other algorithms.
Again this divide-and-conquer algorithm partitions the state $D$ into quadrants, but at this time one of them ($D_{10}$) is empty since $D_{i,j}$ does not make sense when $i>j$.
The quadrant $D_{01}$ depends on the other two.
The algorithm first recursively computes $D_{00}$ and $D_{11}$, then updates $D_{01}$ using the computed values in $D_{00}$ and $D_{11}$, and finally recursively computes $D_{01}$.
Here $D_{01}$ is square, so the recursive computation of $D_{01}$ is almost identical to that in RNA or GAP recurrence (although the labeling of the quadrants is slightly changed): breaking a subtask into four quadrants, recursively solving each of them in the correct order while applying inter-quadrant updates in the middle.
The only difference is when the inter-quadrant updates are processed, each update requires two values, one in $D_{01}$ and another in $D_{00}$ or $D_{11}$.
This is the reason that Parenthesis is 3d while RNA and GAP are 2d.
The correctness of this algorithm can be shown inductively.
%It is easy to check that the values this subregion are finalized, which guarantees the correctness of the algorithm.

\begin{theorem}\label{thm:paren}
The Parenthesis recurrence can be computed in $\Theta(n^3)$ work, optimal symmetric and asymmetric cache complexity of $\displaystyle \Theta\left(\frac{n^3}{B\sqrt{M}}\right)$ and $\displaystyle \Theta\left(\frac{\wcost{}^{1/3} n^3}{B\sqrt{M}}\right)$ respectively, and $O(n^{\log_23})$ depth.
\end{theorem}

\section{2-Knapsack Recurrence}

Given $A_{i}$ and $B_i$ for $0\le i\le n$, the 2-knapsack recurrence computes:
\[D_i=\min_{0\le j\le i}\{A_{j}+B_{i-j}+w(j,i-j,i)\}\]
for $0\le i\le n$.
The cost function $w(j,i-j,i)$ relies on constant input values related on indices $i$, $i-j$ and $j$.
To the best of our knowledge, this recurrence is first discussed in this paper.
We name is the ``2-knapsack recurrence'' since it can be interpreted as the process of finding the optimal strategy in merging two knapsacks, given the optimal local arrangement of each knapsack stored in $A$ and $B$.
Although this recurrence seems trivial, the computation structure of this recurrence actually forms some more complicated DP recurrence.
For example, many problems on trees\footnote{Such problems can be: (1) computing a size-$k$ independent vertex set on a tree that maximizes overall neighbor size, total vertex weights, etc.; (2) tree properties such that the number of subtrees of certain size, tree edit-distance, etc.; (3) many approximation algorithms on tree embeddings of an arbitrary metric~\cite{blelloch2017efficient,blelloch2012parallel}; and many more.} can be solved using dynamic programming, such that the computation essentially applies the 2-knapsack recurrence a hierarchical (bottom-up) manner.

We start by analyzing the lower bound on cache complexity of the 2-knapsack recurrence.
The computational grid has two dimensions, corresponding to $i$ and $j$ in the recurrence.
If we ignore $B$ in the recurrence, then the recurrence is identical to LWS (with no data dependencies), so we can apply the lower bounds in Section~\ref{sec:lws} here.

Note that each update requires two input values $A_{j}$ and $B_{i-j}$, but they are not independent.
When computing a subtask that corresponding to $(i,j)\in[i_0,i_0+n_i]\times[j_0,j_0+n_j]$, the projection sizes on input and output arrays $A$, $B$ and $D$ are no more than $n_j$, $n_i+n_j$ and $n_i$.
This indicates that the computation of this recurrence is a variant of \kdcomp{2}, so we can use the same algorithm discussed in Section~\ref{sec:algorithm}.
\begin{corollary}\label{thm:knapsack}
2-knapsack recurrence can be computed using $O(n^2)$ work, optimal symmetric and asymmetric cache complexity of $\displaystyle \Theta\left(n^2\over B{M}\right)$ and $\displaystyle \Theta\left(\wcost^{1/2}n^2\over B{M}\right)$, and $O(\log^2 n)$ depth.
\end{corollary}



==> table-sublinear-depth.tex <==
\begin{table*}[!ht]
  \centering
  \def\arraystretch{2.5}
    \begin{tabular}{ccccc}
    \toprule
    \multicolumn{1}{c}{\textbf{Recurrence}} & Symmetric I/O cost & Asymetric I/O cost & depth & range of $t$ \\
    \midrule
    LWS & $\displaystyle \Theta\left(\frac{nt}{B}+\frac{nt^2}{B\sqrt{M}}+\frac{n^2}{BM}\right)$ & $\displaystyle \Theta\left(\frac{\wcost{}nt}{B}+\frac{\wcost^{1/3}nt^2}{B\sqrt{M}}+\frac{\wcost^{1/2}n^2}{BM}\right)$ & $\displaystyle O\left(\frac{n}{t}\cdot\log^2 n\right)$ & $t=O(\sqrt{n})$\\
    GAP & $\displaystyle \Theta\left(\frac{n^2t^2}{B}+\frac{n^2t^4}{B\sqrt{M}}+\frac{n^3}{BM}\right)$ & $\displaystyle \Theta\left(\frac{\wcost{}n^2t^2}{B}+\frac{\wcost^{1/3}n^2t^4}{B\sqrt{M}}+\frac{\wcost^{1/2}n^3}{BM}\right)$ & $\displaystyle O\left(\left(\frac{n}{t}\right)^{\log_23}\right)$ & $t=O({n}^{1/4})$\\
    RNA & $\displaystyle \Theta\left(\frac{n^2t^2}{B}+\frac{n^2t^4}{B\sqrt{M}}+\frac{n^4}{BM}\right)$ & $\displaystyle \Theta\left(\frac{\wcost{}n^2t^2}{B}+\frac{\wcost^{1/3}n^2t^4}{B\sqrt{M}}+\frac{\wcost^{1/2}n^4}{BM}\right)$ & $\displaystyle O\left(\left(\frac{n}{t}\right)^{\log_23}\right)$ & $t=O(\sqrt{n})$\\
    Paranthesis & $\displaystyle \Theta\left(\frac{n^2t^2\log n}{B}+\frac{n^3}{B\sqrt{M}}\right)$ & $\displaystyle \Theta\left(\frac{\wcost{}n^2t^2\log n}{B}+\frac{\wcost^{1/3}n^3}{B\sqrt{M}}\right)$ & $\displaystyle \tilde{O}\left(\left(\frac{n}{t}\right)^{\log_23}\right)$ & $t=O((\frac{n}{\log n})^{1/4})$\\
\bottomrule
    \end{tabular}%
  \caption{\label{tbl:table-depth}
  }
\end{table*}%


